Control Regularization for Reduced Variance Reinforcement Learning

Dealing with high variance is a significant challenge in model-free reinforcement learning (RL). Existing methods are unreliable, exhibiting high variance in performance from run to run using different initializations/seeds. Focusing on problems arising in continuous control, we propose a functional regularization approach to augmenting model-free RL. In particular, we regularize the behavior of the deep policy to be similar to a policy prior, i.e., we regularize in function space. We show that functional regularization yields a bias-variance trade-off, and propose an adaptive tuning strategy to optimize this trade-off. When the policy prior has control-theoretic stability guarantees, we further show that this regularization approximately preserves those stability guarantees throughout learning. We validate our approach empirically on a range of settings, and demonstrate significantly reduced variance, guaranteed dynamic stability, and more efficient learning than deep RL alone.

==> sec_algorithm.tex <==
\section{Algorithm}
\label{sec:algorithm}
Our learning algorithm is described in Algorithm \ref{alg:mix_1}. At the high level, the process can be described as:
\begin{itemize}[topsep=-0.1pt, leftmargin=*]
	\itemsep-0.15em
	\item First compute the control prior (Lines 1-2). For robustness, the $\mathcal{H}^{\infty}$ controller can be utilized, though many other choices are possible.
	\item For a given policy iteration, compute the regularization weight, $\lambda$, at each time step using the strategy described in Section 4.2 (Lines 7-9). The algorithm also allows using fixed regularization weight, $\lambda$ (Lines 10-11).
	\item Deploy the mixed policy (\ref{eq:policy_mixed}) on the system, and record the resulting states/action/rewards (Lines 13-15). 
	\item At the end of each policy iteration, update the policy based on the recorded state/action/rewards (Lines 16-18).
\end{itemize}

\begin{algorithm}[tb]
	\caption{Learning Algorithm}\label{alg:mix_1}
	\begin{algorithmic}[1]
		\STATE Obtain initial linearized model $\dot{x} = A x + B u$
		\STATE Compute control prior, $u_{prior}$; Initialize RL policy $\pi_{\theta_0}$
		\STATE Initialize array $\mathcal{D}$ for storing rollout data
		\STATE Set $k=1$ (representing $k^{th}$ policy iteration)
		\WHILE {$k < ~ $Episodes}
		\STATE Evaluate policy $\pi_{\theta_{k-1}}$ at each timestep
		\IF{Using Adaptive Mixing Strategy}
		\STATE At each timestep, compute regularization weight $\lambda$ 
		\STATE{~ for the control prior using the TD-error from (\ref{eq:lambda_td}).}
		\ELSE
		\STATE Set constant regularization weight $\lambda$
		\ENDIF
		\STATE Deploy mixed policy $\pi_{k-1}$ from (\ref{eq:policy_mixed}) to obtain 
		\STATE{~~~~~ rollout of state-action-reward for T timesteps.}
		\STATE{Store resulting data ($s_t, a_t, r_t, s_{t+1}$) in array $\mathcal{D}$.}
		\STATE Using data in $\mathcal{D}$, update policy using any policy 
		\STATE{~~~~~ gradient-based RL algorithm (e.g. DDPG, TRPO)}
		\STATE{~~~~~to obtain $\theta_k$.}
		\STATE $k = k + 1$
		\ENDWHILE
		\STATE \textbf{return} Policy $\pi_{\theta_k}, ~ u_{prior} ~~~~~~~~~~~~~~~~ \rhd$ Overall controller
	\end{algorithmic}
\end{algorithm}


